DelTA: Discriminative Token Credit Assignment for Reinforcement Learning from Verifiable Rewards

Reinforcement learning from verifiable rewards (RLVR) has emerged as a central technique for improving the reasoning capabilities of large language models. Despite its effectiveness, how response-level rewards translate into token-level probability changes remains poorly understood. We introduce a discriminator view of RLVR updates, showing that the policy-gradient update direction implicitly acts as a linear discriminator over token-gradient vectors and thereby determines which token probabilities are increased or decreased during learning. Under standard sequence-level RLVR, this discriminator is constructed from positive- and negative-side centroids formed by advantage-weighted averaging of token-gradient vectors. However, such centroid construction can be dominated by shared high-frequency patterns, such as formatting tokens, diluting sparse yet discriminative directions that better distinguish high-reward responses from low-reward ones. To address this limitation, we propose $\textbf{DelTA}$, a discriminative token credit assignment method that estimates token coefficients to amplify side-specific token-gradient directions and downweight shared or weakly discriminative ones. These coefficients reweight a self-normalized RLVR surrogate, making the effective side-wise centroids more contrastive and thereby reshaping the RLVR update direction. On seven mathematical benchmarks, DelTA outperforms the strongest same-scale baselines by 3.26 and 2.62 average points on Qwen3-8B-Base and Qwen3-14B-Base, respectively. Additional results on code generation, a different backbone, and out-of-domain evaluations further demonstrate the generalization ability of DelTA.

==> tabs/l2_tab.tex <==
\begin{table}[t]
\centering
\caption{
Robust within-side centroid ablation on representative mathematical reasoning benchmarks.
DAPO corresponds to the original squared-\(\ell_2\) side-wise centroid implied by the local update, while the \(\ell_2\)-centroid variant replaces it with a robust within-side centroid estimator without using the opposite-side centroid.
The best results are in \textbf{bold}.
}
\label{tab:l2}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.06}

\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}p{0.34\linewidth}*{5}{>{\centering\arraybackslash}X}@{}}
\toprule
\textbf{Method}
& AIME25
& AIME26
& HMMT25
& HMMT26
& Avg. \\
\midrule

\rowcolor{cyan!10}
\bodystrut \textbf{DelTA}
& \textbf{26.46} & \textbf{28.12} & \textbf{18.54} & \textbf{20.27} & \textbf{23.27} \\

\midrule
\bodystrut DAPO (\(\ell^2_2\)-centroid)
& 23.33  & 24.17 & 12.08 & 16.86 & 19.05 \\
\bodystrut \(\ell_2\)-centroid
& 19.38 & 20.00 & 8.54 & 14.58 & 15.60 \\

\bottomrule
\end{tabularx}
\end{table}
